Deep Neural Network approaches for Analysing Videos of Music Performances

This paper presents a framework to automate the labelling process for gestures in musical performance videos with a 3D Convolutional Neural Network (CNN). While this idea was proposed in a previous study, this paper introduces several novelties: (i) Presents a novel method to overcome the class imbalance challenge and make learning possible for co-existent gestures by batch balancing approach and spatial-temporal representations of gestures. (ii) Performs a detailed study on 7 and 18 categories of gestures generated during the performance (guitar play) of musical pieces that have been video-recorded. (iii) Investigates the possibility to use audio features. (iv) Extends the analysis to multiple videos. The novel methods significantly improve the performance of gesture identification by 12 %, when compared to the previous work (51 % in this study over 39 % in previous work). We successfully validate the proposed methods on 7 super classes (72 %), an ensemble of the 18 gestures/classes, and additional videos (75 %).

==> tables/class_distribution_18_old.tex <==
\begin{table}[!t]
    \small
    \footnotesize
\centering

\caption{Number of frames where each of the classes are present per video}
\label{tab:18classdistribution_old}
   % \begin{adjustbox}{width=\textwidth}
\begin{tabular}{lrrrr}
\hline
\textbf{Class}               & \textbf{video-1} & \textbf{video-2} & \textbf{video-3} & \textbf{video-4} \\ \hline
\hline
Facial expression            & 217              & 62               & 195              & 121              \\
Nodding                      & 86               & 48               & 59               & 80               \\
Right hand round             & 73               & 35               & 92               & 71               \\
Expressive shoulder movement & 127              & 119              & 132              & 249              \\
Left hand gesture            & 73               & 24               & 57               & 79               \\
Lifting head                 & 92               & 89               & 128              & 112              \\
Minimal movement             & 0                & 251              & 255              & 269              \\
Eyes closed                  & 78               & 14               & 79               & 70               \\
Vibrato                      & 27               & 30               & 43               & 33               \\
Expressive preparation       & 55               & 0                & 75               & 38               \\
Freeze                       & 53               & 33               & 118              & 101              \\
Expressive head movement     & 15               & 20               & 20               & 34               \\
Frowning                     & 277              & 76               & 265              & 234              \\
Physical energy              & 53               & 8                & 0                & 7                \\
Upbeat in head movement      & 0                & 4                & 8                & 6                \\
Repositioning guitar         & 0                & 12               & 40               & 90               \\
Sympathetic body movement    & 0                & 0                & 0                & 0                \\
Normal play                  & 273              & 135              & 255              & 166             \\
\hline
\end{tabular}
%\end{adjustbox}
\end{table}

==> tables/gesture_occurancies_old.tex <==
\begin{table}[!t]
    \small
    \footnotesize
\centering

\caption{Number of occurrences for each gesture for each video - 18 classes}
\label{tab:gesture_occurrences_18_old}
   % \begin{adjustbox}{width=\textwidth}
\begin{tabular}{lrrrr}
\hline
\textbf{Class}               & \textbf{video-1} & \textbf{video-2} & \textbf{video-3} & \textbf{video-4} \\ \hline
\hline
Facial expression            & 42              & 14               & 17              & 13              \\
Nodding                      & 59               & 28               & 46               & 55               \\
Right hand round             & 18               & 11               & 20               & 20               \\
Expressive shoulder movement & 24              & 19              & 20              & 36              \\
Left hand gesture            & 21               & 8               & 16               & 16               \\
Lifting head                 & 22               & 20               & 22              & 24              \\
Minimal movement             & 9                & 18              & 10              & 11              \\
Eyes closed                  & 22               & 4               & 12               & 17               \\
Vibrato                      & 17               & 15               & 23               & 20               \\
Expressive preparation       & 17               & 0                & 17               & 10               \\
Freeze                       & 13               & 12               & 23              & 22              \\
Expressive head movement     & 8               & 5               & 7               & 7               \\
Frowning                     & 62              & 20               & 66              & 55              \\
Physical energy              & 53               & 8                & 0                & 7                \\
Upbeat in head movement      & 5                & 2                & 6                & 4               \\
Repositioning guitar         & 5                & 3               & 12               & 25               \\
Sympathetic body movement    & 0                & 0                & 0                & 0                \\
Normal play                  & -              & -              & -              & -             \\
\hline
\end{tabular}
%\end{adjustbox}
\end{table}


